Neumann Data and Second Variation Formula of Renormalized Area for Conformally Compact Static Spaces

In this paper, we derive the first and second variation formulas for the renormalized area for static Einstein spaces along a specific direction, demonstrating that the negativity of the Neumann data implies instability. Consequently, we obtain a rigidity result for the case when the conformal boundary is a warped product torus, which strengthens the result presented in \cite{GSW}.

==> ref2.tex <==
\begin{thebibliography}{99}

\bibitem{Am}
L. Ambrozio,
\textit{On static three-manifolds with positive scalar curvature},
J. Differential Geom. \textbf{107} (2017), no. 1, 1--45.

\bibitem{an2020ellipticity}
Z. An,
\textit{Ellipticity of Bartnik boundary data for stationary vacuum spacetimes},
Comm. Math. Phys. \textbf{373} (2020), no. 3, 859--906.

\bibitem{an2021initial}
Z. An and M. T. Anderson,
\textit{The initial boundary value problem and quasi-local Hamiltonians in General Relativity},
Classical Quantum Gravity \textbf{38} (2021), no. 15, 154001.

\bibitem{Anderson2000}
M. T. Anderson,
\textit{On the Structure of Solutions to the Static Vacuum Einstein Equations},
Ann. Henri Poincaré \textbf{1} (2000), no. 5, 995--1042.

\bibitem{Ander}
M. T. Anderson,
\textit{Static Vacuum Einstein Metrics on Bounded Domains},
Ann. Henri Poincaré \textbf{16} (2015), 2265--2302.

\bibitem{baltazar2018remarks}
H. Baltazar and E. Ribeiro,
\textit{Remarks on critical metrics of the scalar curvature and volume functionals on compact manifolds with boundary},
Pacific J. Math. \textbf{297} (2018), no. 1, 29--45.

\bibitem{barzegar2020remarks}
H. Barzegar, P. T. Chruściel, M. Hörzinger, M. Maliborski, and L. Nguyen,
\textit{Remarks on the energy of asymptotically Horowitz-Myers metrics},
Phys. Rev. D \textbf{101} (2020), no. 2, 024007.

\bibitem{besse2007einstein}
A. L. Besse,
\textit{Einstein manifolds},
Springer, 2007.

\bibitem{BF}
S. Borghini and M. Fogagnolo,
\textit{Comparison geometry for substatic manifolds and a weighted Isoperimetric Inequality},
arXiv:2307.14618 (2023).

\bibitem{boucher1984uniqueness}
W. Boucher, G. W. Gibbons, and G. T. Horowitz,
\textit{Uniqueness theorem for anti-de Sitter spacetime},
Phys. Rev. D \textbf{30} (1984), no. 12, 2447.

\bibitem{Bo}
J. P. Bourguignon,
\textit{Une stratification de l'espace des structures riemanniennes},
Compositio Math. \textbf{30} (1975), 1--41.

\bibitem{SB}
S. Brendle,
\textit{Constant mean curvature surfaces in warped product manifolds},
Publ. Math. Inst. Hautes Études Sci. \textbf{117} (2013), 247--269.

\bibitem{BH}
S. Brendle and P. K. Hung,
\textit{Systolic inequalities and the Horowitz-Myers conjecture},
arXiv:2406.04283 (2024).

\bibitem{bunting1987nonexistence}
G. L. Bunting and A. K. M. Masood-ul-Alam,
\textit{Nonexistence of multiple black holes in asymptotically Euclidean static vacuum space-time},
Gen. Relativity Gravitation \textbf{19} (1987), 147--154.

\bibitem{CG2}
M. Cai and G. J. Galloway,
\textit{Boundaries of zero scalar curvature in the AdS/CFT correspondence},
Adv. Theor. Math. Phys. \textbf{3} (1999), 1769--1783.

\bibitem{chang2011fractional}
S.-Y. A. Chang and M. del Mar González,
\textit{Fractional Laplacian in conformal geometry},
Adv. Math. \textbf{226} (2011), no. 2, 1410--1432.

\bibitem{chang2018compactness}
S.-Y. A. Chang and Y. Ge,
\textit{Compactness of conformally compact Einstein manifolds in dimension 4},
Adv. Math. \textbf{340} (2018), 588--652.

\bibitem{CG}
J. Cheeger and D. Gromoll,
\textit{The splitting theorem for manifolds of nonnegative Ricci curvature},
J. Differential Geom. \textbf{6} (1971), 119--128.

\bibitem{Co}
J. Corvino,
\textit{Scalar curvature deformation and a glueing construction for the Einstein constraint equations},
Comm. Math. Phys. \textbf{214} (2000), 137--189.

\bibitem{DJ}
S. Dutta and M. Javaheri,
\textit{Rigidity of conformally compact manifolds with the round sphere as the conformal infinity},
Adv. Math. \textbf{224} (2010), no. 2, 525--538.

\bibitem{EH}
G. F. R. Ellis and S. W. Hawking,
\textit{The Large Scale Structure of Space-Time},
Cambridge Univ. Press, 1973.

\bibitem{FF}
H. Fédérer and W. H. Fleming,
\textit{Normal and Integral Currents},
Ann. of Math. \textbf{72} (1960), 458.

\bibitem{FM}
A. Fischer and J. Marsden,
\textit{Linearization stability of nonlinear partial differential equations},
Proc. Sympos. Pure Math. \textbf{27} (1975), 219--262.

\bibitem{Ga}
G. J. Galloway,
\textit{On the topology of black holes},
Comm. Math. Phys. \textbf{151} (1993), 53--66.

\bibitem{Ga1}
G. Galloway,
\textit{Maximum Principles for Null Hypersurfaces and Null Splitting Theorems},
Ann. Henri Poincaré \textbf{1} (2000), 543--567.

\bibitem{GSW}
G. J. Galloway, S. Surya, and E. Woolgar,
\textit{On the Geometry and Mass of Static, Asymptotically AdS Spacetimes, and the Uniqueness of the AdS Soliton},
Comm. Math. Phys. \textbf{241} (2002), 1--25.

\bibitem{horowitz1998ads}
G. T. Horowitz and R. C. Myers,
\textit{AdS-CFT correspondence and a new positive energy conjecture for general relativity},
Phys. Rev. D \textbf{59} (1998), no. 2, 026005.

\bibitem{israel1968event}
W. Israel,
\textit{Event horizons in static electrovac space-times},
Comm. Math. Phys. \textbf{8} (1968), 245--260.

\bibitem{Ko}
O. Kobayashi,
\textit{A differential equation arising from scalar curvature function},
J. Math. Soc. Japan \textbf{34} (1982), no. 4, 665--675.

\bibitem{La}
J. Lafontaine,
\textit{Sur la geometrie d'une generalisation de l'equation d'Obata},
J. Math. Pures Appl. \textbf{62} (1983), 63--72.

\bibitem{Da}
D. Lee,
\textit{Geometric Relativity},
Graduate Studies in Mathematics, 2019.

\bibitem{Li}
P. Li,
\textit{Geometric Analysis},
Cambridge Univ. Press, 2012.

\bibitem{LX}
J. Li and C. Xia,
\textit{An integral formula and its applications on sub-static manifolds},
J. Differential Geom. \textbf{113} (2019), no. 3, 493--518.

\bibitem{Pe}
P. Petersen,
\textit{Riemannian Geometry},
Springer, 2006.

\bibitem{qing2013note}
J. Qing and W. Yuan,
\textit{A note on static spaces and related problems},
J. Geom. Phys. \textbf{74} (2013), 18--27.

\bibitem{robinson1977simple}
D. C. Robinson,
\textit{A simple proof of the generalization of Israel's theorem},
Gen. Relativity Gravitation \textbf{8} (1977), 695--698.

\bibitem{SY}
R. Schoen and S. T. Yau,
\textit{Existence of incompressible minimal surfaces and the topology of three dimensional manifolds with non-negative scalar curvature},
Ann. of Math. \textbf{110} (1979), no. 1, 127--142.

\bibitem{shi2005rigidity}
Y. Shi and G. Tian,
\textit{Rigidity of asymptotically hyperbolic manifolds},
Comm. Math. Phys. \textbf{259} (2005), no. 3, 545--559.

\bibitem{shen1997note}
Y. Shen,
\textit{A note on Fischer-Marsden's conjecture},
Proc. Amer. Math. Soc. \textbf{125} (1997), no. 3, 901--905.

\bibitem{Wald2010general}
R. M. Wald,
\textit{General relativity},
Univ. Chicago Press, 2010.

\bibitem{Wa}
X. Wang,
\textit{The Mass of Asymptotically Hyperbolic Manifolds},
J. Differential Geom. \textbf{57} (2001), 273--299.

\bibitem{Wa2}
X. Wang,
\textit{On Conformally Compact Einstein Manifolds},
Math. Res. Lett. \textbf{8} (2001), 671--688.

\bibitem{wang2005uniqueness}
X. Wang,
\textit{On the uniqueness of the AdS spacetime},
Acta Math. Sinica \textbf{21} (2005), 917--922.

\bibitem{wang2024riccati}
Z. Wang,
\textit{Riccati Equation for Static Spaces and its Applications},
arXiv:2408.12180 (2024).

\bibitem{Witten1998}
E. Witten,
\textit{Anti-de Sitter space and holography},
Adv. Theor. Math. Phys. \textbf{2} (1998), no. 2, 253--291.

\bibitem{WY}
E. Witten and S. Yau,
\textit{Connectedness of the boundary in the AdS/CFT correspondence},
Adv. Theor. Math. Phys. \textbf{3} (1999), 1635--1655.

\bibitem{Wo}
E. Woolgar,
\textit{The rigid Horowitz-Myers conjecture},
J. High Energy Phys. \textbf{2017} (2017), no. 1--27.

\bibitem{qing2003rigidity}
J. Qing,
\textit{On the rigidity for conformally compact Einstein manifolds},
Int. Math. Res. Not. \textbf{2003} (2003), no. 21, 1141--1153.

\bibitem{graham1999conformal}
C. R. Graham and E. Witten,
\textit{Conformal anomaly of submanifold observables in AdS/CFT correspondence},
Nuclear Phys. B \textbf{546} (1999), no. 1-2, 52--64.

\bibitem{Graham2000}
C. R. Graham,
\textit{Volume and Area Renormalizations for Conformally Compact Einstein Metrics},
Rend. Circ. Mat. Palermo \textbf{2} (2000), no. Suppl. 63, 31--42.

\bibitem{alexakis2010renormalized}
S. Alexakis and R. Mazzeo,
\textit{Renormalized area and properly embedded minimal surfaces in hyperbolic 3-manifolds},
Comm. Math. Phys. \textbf{297} (2010), no. 3, 621--651.

\bibitem{albin2009renormalizing}
P. Albin,
\textit{Renormalizing curvature integrals on Poincaré-Einstein manifolds},
Adv. Math. \textbf{221} (2009), no. 1, 140--169.

\bibitem{anderson1982complete}
M. T. Anderson,
\textit{Complete minimal varieties in hyperbolic space},
Invent. Math. \textbf{69} (1982), no. 3, 477--494.

\bibitem{anderson1983complete}
M. T. Anderson,
\textit{Complete minimal hypersurfaces in hyperbolic n-manifolds},
Comment. Math. Helv. \textbf{58} (1983), 264--290.

\bibitem{hardt1987regularity}
R. Hardt and F.-H. Lin,
\textit{Regularity at infinity for area-minimizing hypersurfaces in hyperbolic space},
Invent. Math. \textbf{88} (1987), no. 1, 217--224.

\bibitem{lin1989dirichlet}
F. H. Lin,
\textit{On the Dirichlet problem for minimal graphs in hyperbolic space},
Invent. Math. \textbf{96} (1989), no. 3, 593--612.

\bibitem{marx2021variations}
J. Marx-Kuo,
\textit{Variations of renormalized volume for minimal submanifolds of Poincaré-Einstein manifolds},
arXiv:2111.04294 (2021).

\bibitem{graham1999volume}
C. R. Graham,
\textit{Volume and area renormalizations for conformally compact Einstein metrics},
arXiv:math/9909042 (1999).

\bibitem{Lee1994TheSO}
J. M. Lee,
\textit{The spectrum of an asymptotically hyperbolic Einstein manifold},
Comm. Anal. Geom. \textbf{3} (1994), 253--271.

\bibitem{Fdrer1960NormalAI}
H. Fédérer and W. H. Fleming,
\textit{Normal and Integral Currents},
Ann. of Math. \textbf{72} (1960), 458.

\bibitem{Allard1972OnTF}
W. K. Allard,
\textit{On the first variation of a varifold},
Ann. of Math. \textbf{95} (1972), 417--491.

\bibitem{Tonegawa1996ExistenceAR}
Y. Tonegawa,
\textit{Existence and regularity of constant mean curvature hypersurfaces in hyperbolic space},
Math. Z. \textbf{221} (1996), 591--615.

\end{thebibliography}
